CerebroSim: Scalable Whole-Brain Simulator at 100-Trillion-Synapse Scale on the LineShine Supercomputer

Building executable brain models is essential for moving neuroscience from description to mechanism and prediction. Human-brain-scale spiking simulation is constrained by highly irregular communication, multithreaded spike delivery, and the memory cost of sparse connectivity. We present CerebroSim, a scalable framework for whole-brain simulation. CerebroSim combines Delay-aware Spike Broadcast (DSB) for aggregated delay-aware communication, Race-free Synaptic Dynamics Computation (RSDC) for lock/atomic-free multithreaded delivery with HBM-aware optimization, and Sparse Synapse Storage Compression (3SC) for compact indexing with deterministic synapse regeneration. Using a model derived from magnetic resonance imaging and diffusion-weighted imaging, CerebroSim simulates 86 billion neurons and 100 trillion synapses on 18,432 nodes across 11.2 million cores of the LineShine Supercomputer, sustaining 24.44 PFlop/s, 91% weak-scaling efficiency, and 94% strong-scaling efficiency. This capability makes biologically constrained human-brain models practical for mechanistic studies of brain disorders and controlled in silico testing of intervention hypotheses.

==> sections/section91_acknowledgments.tex <==
% 致谢（投稿阶段暂不启用：main.tex 里的 \input 已注释掉）
% 需要时：把正文补在下面，并在 main.tex 里取消 \input{sections/section91_acknowledgments} 的注释。
% 注意：源稿 20260415_CerebroSim_GB/text/Section8_Implications.tex 没有致谢内容，
% 原稿的致谢段全部是注释状态，本稿也未迁入任何致谢文字。

\section*{Acknowledgments}

% TODO: 在此填写资助信息与致谢（基金编号、计算资源提供方等）。

